Using Herschel and Planck observations to delineate the role of magnetic fields in molecular cloud structure

We present a study of the relative orientation between the magnetic field projected onto the plane of sky ($B_{\perp}$) on scales down to 0.4 pc, inferred from the polarized thermal emission of Galactic dust observed by Planck at 353 GHz, and the distribution of gas column density ($N_{\rm H}$) structures on scales down to 0.026 pc, derived from the observations by Herschel in submillimeter wavelengths, toward ten nearby ($d$$<$450 pc) molecular clouds. Using the histogram of relative orientation technique in combination with tools from circular statistics, we found that the mean relative orientation between $N_{\rm H}$ and $B_{\perp}$ toward these regions increases progressively from 0\deg, where the $N_{\rm H}$ structures lie mostly parallel to $B_{\perp}$, with increasing $N_{\rm H}$, in many cases reaching 90\deg, where the $N_{\rm H}$ structures lie mostly perpendicular to $B_{\perp}$. We also compared the relative orientation between $N_{\rm H}$ and $B_{\perp}$ and the distribution of $N_{\rm H}$, which is characterized by the slope of the tail of the $N_{\rm H}$ probability density functions (PDFs). We found that the slopes of the $N_{\rm H}$ PDF tail are steepest in regions where $N_{\rm H}$ and $B_{\perp}$ are close to perpendicular. This coupling between the $N_{\rm H}$ distribution and the magnetic field suggests that the magnetic fields play a significant role in structuring the interstellar medium in and around molecular clouds. However, we found no evident correlation between the star formation rates, estimated from the counts of young stellar objects, and the relative orientation between $N_{\rm H}$ and $B_{\perp}$ in these regions.

==> PlanckTable.tex <==
%Planck table template file, to be used with A&A style and Planck.tex to produce Planck tables %  for publication.
%
% version 11 September 2011 ---  CRL

\begin{table*}[tmb]                 % table* is a two-column table.  Drop the * for one column.
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{}                          % Caption goes here.
\label{}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{+} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{                            % Template goes here.
\noalign{\doubleline}
                                    % Table headings go here.
\noalign{\vskip 3pt\hrule\vskip 5pt}
                                    % Body of table goes here.
\noalign{\vskip 5pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
\tablenote a Footnote a.\par
\tablenote b Footnote b.\par
\endgroup
\end{table*}                        % table* is a two-column table.  Drop the * for one column.


==> polar_definitions.tex <==
%This is a proposal for homogeneous polarization notations in the
%Planck PIP papers.
% They are the same as in Fig 14 of the paper by Levrier, except for B
%Feel free to add to it if you need more, or propose for changes.
%JPB Jan 21 2013

%=== Stokes parameters
\newcommand{\StokesI}{\rm I}                    %Intensity
\newcommand{\StokesQ}{\rm Q}                    %Q
\newcommand{\StokesU}{\rm U}                    %U
%=== Polarization quantities
\newcommand{\polint}{\rm P}                     %polarization intensity
\newcommand{\polfrac}{\rm p}                    %polarization fraction
\newcommand{\polang}{\rm \psi}                  %polarization angle
\newcommand{\sigpolfrac}{\rm \sigma_{\polfrac}}   %polarization fraction uncertainty
\newcommand{\sigpolang}{\rm \sigma_{\polang}}     %polarization angle uncertainty
\newcommand{\polangsky}{\rm \gamma}             %B-field angle wrt sky plane
\newcommand{\DeltaAng}{\Delta \polang}          %polarization angle structure function
%=== Stockes parameters variances
\newcommand{\sigII}{\rm \sigma_{II}}            % Intensity sqrt(variance)
\newcommand{\sigQQ}{\rm \sigma_{QQ}}            % Q sqrt(variance)
\newcommand{\sigUU}{\rm \sigma_{UU}}            % U sqrt(variance)
\newcommand{\sigIQ}{\rm \sigma_{IQ}}            % IQ sqrt(covariance)
\newcommand{\sigIU}{\rm \sigma_{IU}}            % IU sqrt(covariance)
\newcommand{\sigQU}{\rm \sigma_{QU}}            % QU sqrt(covariance)
\newcommand{\sigsquareII}{\rm \sigma^2_{II}}    % Intensity variance
\newcommand{\sigsquareQQ}{\rm \sigma^2_{QQ}}    % Q variance
\newcommand{\sigsquareUU}{\rm \sigma^2_{UU}}    % U variance
\newcommand{\sigsquareIQ}{\rm \sigma^2_{IQ}}    % IQ covariance
\newcommand{\sigsquareIU}{\rm \sigma^2_{IU}}    % IU covariance
\newcommand{\sigsquareQU}{\rm \sigma^2_{QU}}    % QU covariance
%=== B field
\newcommand{\Borth}{\rm B_{\perp}}              %B orthogonal to LOS (ie, Plane of sky)
\newcommand{\Bpar}{\rm B_{\parallel}}           %B parallel to LOS


